Covariance Steering of Discrete-Time Stochastic Linear Systems Based on Distribution Distance Terminal Costs

We consider a class of stochastic optimal control problems for discrete-time stochastic linear systems which seek for control policies that will steer the probability distribution of the terminal state of the system close to a desired Gaussian distribution. In our problem formulation, the closeness between the terminal state distribution and the desired (goal) distribution is measured in terms of the squared Wasserstein distance which is associated with a corresponding terminal cost term. We recast the stochastic optimal control problem as a finite-dimensional nonlinear program and we show that its performance index can be expressed as the difference of two convex functions. This representation of the performance index allows us to find local minimizers of the original nonlinear program via the so-called convex-concave procedure [1]. Subsequently, we consider a similar problem but this time we use a terminal cost that corresponds to the KL divergence. Finally, we present non-trivial numerical simulations to demonstrate the proposed techniques and compare them in terms of computation time.

==> cvx-cost.tex <==
\revision{
If terminal cost in optimal control problem is picked as convex cost function (\ref{cvx-cost-metrix}) then problem becomes convex. Since we already showed that $\E{\sum_{k=0}^{N-1} u_k^T u_k}{}$ yields a convex function we need to show that rest is also convex.
}
\begin{multline}
    \mathcal{D}(\mathcal{N}_N, \mathcal{N}_d) = \lVert \bs{F} (\bs{\Gamma} \mu_0 +\bs{H_u u_{ff}})  -\mu_d \rVert_2^2 + \\
    \lVert (\bs{F} (\bs{I} + \bs{H_u \Theta}) \Bar{V}^T \Bar{D}^{1/2}) - V_d D_d^{1/2} \rVert_{F}^{2}
\end{multline}
\revision{
where $\Bar{V}^T \Bar{D} \Bar{V} = \Bar{S}$ and $V_d^T D_d V_d = S_d$ are eigenvalue decompositions.
}


==> gradient.tex <==
Convex-concave procedure(CCP)\cite{ccp} is an iterative technique to find local optima of non-convex optimization problems. CCP is based on iterative convexification of objective and constraints and solving convex subproblem. Convexification is done by taking linear approximation concave part part of the function to be convexified. In our case 

Most of the first order solvers require analytical expression of the gradient of objective function and constraints, however one of the decision variable is a matrix thus it requires matrix calculus to derive derivatives $J$ with respect to $K$. We derived these derivatives by taking differential of  
based on jacobian identification rule \cite{kron-product}. Derivation of gradients are provided in the supplementary material.

